Intercusp Geodesics and Cusp Shapes of Fully Augmented Links

We study the geometry of fully augmented link complements in $S^3$ by looking at their link diagrams. We extend the method introduced by Thistlethwaite and Tsvietkova to fully augmented links and define a system of algebraic equations in terms of parameters coming from edges and crossings of the link diagrams. Combining it with the work of Purcell, we show that the solutions to these algebraic equations are related to the cusp shapes of fully augmented link complements. As an application we use the cusp shapes to study the commensurability classes of fully augmented links.

==> bowtie.tex <==
\begin{tikzpicture}[thick,scale=0.8, every node/.style={transform shape}]
 %\draw[light gray](0,0) grid (5,5);
 \draw [red, ultra thick] (0,0) -- (1,2);
 \draw[red, ultra thick] (0,0) -- (2,0);
 \draw[red, ultra thick] (2,0) -- (1,2);


 \draw[red, ultra thick] (1,2) -- (0,4);
 \draw[red, ultra thick] (1,2) -- (2,4);
\draw[red, ultra thick] (0,4) -- (2,4);

 \fill [gray!30] (1,2) -- (0,4) -- (2,4);
 \fill [gray!30] (1,2) -- (0,0) -- (2,0);
  \fill  (0,0) circle (.1cm);
 \fill  (2,0) circle (.1cm);
 \fill  (0,4) circle (.1cm);
 \fill  (2,4) circle (.1cm);
 \fill  (1,2) circle (.1cm);
 
 %\draw[light gray](0,0) grid (5,5);
 \draw [red, ultra thick] (3,0) -- (4,2);
 \draw[red, ultra thick] (3,0) -- (5,0);
 \draw[red, ultra thick] (5,0) -- (4,2);


 \draw[red, ultra thick] (4,2) -- (3,4);
 \draw[red, ultra thick] (4,2) -- (5,4);
\draw[red, ultra thick] (3,4) -- (5,4);

 \fill [gray!30] (4,2) -- (3,4) -- (5,4);
 \fill [gray!30] (4,2) -- (3,0) -- (5,0);
  \fill  (3,0) circle (.1cm);
 \fill  (5,0) circle (.1cm);
 \fill  (3,4) circle (.1cm);
 \fill  (5,4) circle (.1cm);
 \fill  (4,2) circle (.1cm);

 \node at (.3,3.3) {\large$\vee$}; 
 \node at (.3,.7) {\large$\wedge$};
\node at (1.7,3.3) {\large$\vee$}; 
\node at (1.7,3.1) {\large$\vee$};  

\node at (1.7,.7) {\large$\wedge$}; 
\node at (1.7,.9) {\large$\wedge$};  
\node at (1,4)
 {\large$\textgreater$};
 \node at (1.2,4)
 {\large$\textgreater$};
\node at (1.4,4)
 {\large$\textgreater$}; 
 
 \node at (1,0)
 {\large$\textgreater$};
 \node at (1.2,0)
 {\large$\textgreater$};
\node at (1.4,0)
 {\large$\textgreater$}; 
 \node at (1,3) {$A$};
 \node at (1,1) {$A$};
 
 
 \node at (3.3,3.3) {\large$\bigtriangledown $}; 
 \node at (3.3,.7) {\large$\bigtriangleup $};
\node at (4.7,3.3) {\large$\bigtriangledown $}; 
\node at (4.7,3.1) {\large$\bigtriangledown $};  

\node at (4.7,.7) {\large$\bigtriangleup $}; 
\node at (4.7,.9) {\large$\bigtriangleup $};  
\node at (4,4)
 {\large$\rhd∗$};
 \node at (4.2,4)
 {\large$\rhd∗$};
\node at (4.4,4)
 {\large$\rhd∗$}; 
 
 \node at (4,0)
 {\large$\rhd∗$};
 \node at (4.2,0)
 {\large$\rhd∗$};
\node at (4.4,0)
 {\large$\rhd∗$}; 
 \node at (4,3) {$B$};
 \node at (4,1) {$B$};
 
 

==> sign.tex <==
\begin{tikzpicture}
\draw

